The JHU-Microsoft Submission for WMT21 Quality Estimation Shared Task

This paper presents the JHU-Microsoft joint submission for WMT 2021 quality estimation shared task. We only participate in Task 2 (post-editing effort estimation) of the shared task, focusing on the target-side word-level quality estimation. The techniques we experimented with include Levenshtein Transformer training and data augmentation with a combination of forward, backward, round-trip translation, and pseudo post-editing of the MT output. We demonstrate the competitiveness of our system compared to the widely adopted OpenKiwi-XLM baseline. Our system is also the top-ranking system on the MT MCC metric for the English-German language pair.

==> source/experiment-new.tex <==
\section{Experiment}

\subsection{Setup}
\begin{table*}[]
\centering
\scalebox{0.9}{\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Language Pair} & \textbf{Synthesis Method} & \textbf{Data Source}                         & \textbf{\# Triplets} \\ \midrule
English-German         & src-mt-tgt                & WMT20 en-de parallel data                    & 44.2M                \\
English-German         & src-mt1-mt2               & WMT20 en-de parallel data cleaned            & 36.1M                \\
English-German         & bt-rt-tgt                 & 10M sample from newscrawl2020                & 10.0M                \\
English-German         & bt-noisy-tgt              & 10M sample from newscrawl2020                & 10.0M                \\
English-Chinese        & src-mt-tgt                & shared task en-zh parallel                   & 20.3M                \\
English-Chinese        & MVPPE                     & shared task en-zh parallel                   & 20.3M                \\
Romanian-English       & src-rt-ft                 & shared task ro-en parallel                   & 3.09M                \\
Romanian-English       & MVPPE                     & shared task ro-en parallel                   & 3.09M                \\
Russian-English        & src-rt-ft                 & shared task ru-en parallel                   & 2.32M                \\
Estonian-English       & src-rt-ft                 & shared task et-en parallel                   & 880K                 \\
Nepalese-English       & src-rt-ft                 & shared task ne-en parallel                   & 498K                 \\
Pashto-English         & src-rt-ft                 & WMT20 Parallel Corpus Filtering Task         & 347K                 \\ \bottomrule
\end{tabular}}
\caption{Source and statistics of datasets used for our synthetic finetuning experiments. \label{tab:data}}
\end{table*}

\begin{figure*}
\centering
\includegraphics[scale=0.6]{figures/main.pdf}
\caption{Target MCC results on \texttt{test20} dataset for all language pairs we submitted systems for (except for ps-en which is not included in \texttt{test20}).\label{fig:main}}
\end{figure*}

% Data
We follow the data split on human post-edited data as determined by the task organizers and use \texttt{test20} as the devtest for our system development purposes.
Apart from the human post-edited data provided by the task organizers, we also used some extra data for synthetic finetuning.
Table \ref{tab:data} shows the source and statistics of the data that's been used for our synthetic finetuning experiments.
For stage 1 LevT translation training, we always use the same parallel data that is used to train the MT systems provided by the shared task.

For the only language pair where we applied the \textbf{src-mt1-mt2} synthetic finetuning, we used the WMT19 Facebook's winning system \cite{ng-etal-2019-facebook} to generate the higher-quality translation \textbf{mt2}.
For both \textbf{src-mt-tgt} and \textbf{src-mt1-mt2}, we used the system provided by the shared task to generate the MT output in the pseudo translation triplet.
For the Levenshtein Transformer in \textbf{bt-noisy-tgt}, we used a Levenshtein Transformer model trained from scratch (without M2M initialization).
For all the other forward/backward/round-trip translations, we used M2M-mid (1.2B parameters) model to generate the necessary outputs.

% Hyperparameters
All of our experiments uses Adam optimizer \cite{DBLP:journals/corr/KingmaB14} with linear warmup and \texttt{inverse-sqrt} scheduler.
For stage 1, we use the same hyperparameters as \citet{DBLP:conf/nips/GuWZ19} for LevT translation training, but use a smaller learning rate of 2e-5 to avoid overfitting for all to-English language pairs.
For stage 2 and beyond, we stick to the learning rate of 2e-5 and perform early-stopping based on the loss function on the development set. We also experiment with label balancing factor $\sigma=1.0$ and $\sigma=3.0$ for each language pair and pick the one that works the best on devtest data.
We find the QE task performance to be quite sensitive to $\sigma$ but there is also no universally optimal value for all language pairs.

Our LevT-QE model is implemented based on Fairseq \cite{DBLP:conf/naacl/OttEBFGNGA19}.
We also implemented another TER computation tool\footnote{\texttt{https://github.com/marian-nmt/moses-scorers}} to generate the word-level and subword-level tags that we use as the reference for finetuning, but stick to the original reference tags in the test set for evaluation to avoid potential result mismatch.

\subsection{Results}

Our pre-submission results on \texttt{test20} devtest data is shown in Figure \ref{fig:main}.
We can first observe that for all language pairs except English-Chinese, our LevT QE models perform better than the OpenKiwi-XLM \cite{kepler-etal-2019-openkiwi} baselines that we built on our own.\footnote{We followed their \texttt{xlmroberta.yaml} recipe to build our own baseline systems.}
It is not clear as to why English-Chinese is an outlier, but we suspect it might be related to the fact that the M2M model is not a good translation model on this specific language pair, as reported in \cite{DBLP:journals/corr/abs-2010-11125}.
Among the other language pairs, it should be noted that the benefit of LevT is most significant on the language pairs with a large amount of available parallel data.
This is intuitive, because the less parallel data we have, the less knowledge we can draw out of the LevT training process.
In the extreme case where we have no parallel data at all, all of our knowledge comes from the pre-trained model and human annotation data finetuning, which will reduce to the same model as the baseline.
Finally, our Nelder-Meade ensemble further improves the result by a small but steady margin.

We do not have enough time to run a rigorous comparison for all the explored synthetic finetuning methods before the submission deadline (we will include it in our next draft).
Our general development results indicate that \textbf{src-mt1-mt2} works significantly better than all the other synthetic finetuning methods, which does not improve the result and may even hurt sometimes.
This is different from the experiments shown in \cite{lee-2020-two}, which successfully deployed \textbf{src-mt-tgt}-style synthetic finetuning to improve the performance on the word-level QE task.
Note that the limitation of \textbf{src-mt1-mt2} is also pretty clear: it calls for an existing stronger MT system than the one whose translation quality is being estimated, which is why we did not perform similar synthetic finetuning for the language pairs other than en-de, as there are no clearly stronger publicly available MT models for these language pairs.
In theory, we can produce stronger translations for that purpose by resorting to an online translation system such as Google/Bing Translate, which another team used in their 2020 participation \cite{wang-etal-2020-hw}, but those models are not publicly available, hence making the submission results hard to reproduce.
To verify \textbf{src-mt1-mt2} does work beyond en-de language pair, we plan to build contrastive systems that take advantage of the online systems to build synthetic finetuning data.


==> source/method.arxiv.tex <==
\section{Method}

Our system building pipeline is consisted of three different stages:
\begin{itemize} \itemsep -2pt
	\item \textbf{Stage 1}: Training LevT for translation
	\item \textbf{Stage 2 (Optional)}: Finetuning LevT on synthetic post-editing triplets
	\item \textbf{Stage 3}: Finetuning LevT on human post-editing triplets
\end{itemize}
We start by introducing the architecture we use and then describe each stage of our training process.

\subsection{Levenshtein Transformer}

% pasted from the EMNLP submission
The Levenshtein Transformer \cite[LevT,][]{DBLP:conf/nips/GuWZ19} is a non-autoregressive NMT architecture that generates translations by iteratively applying Longest Common Subsequence (LCS) edits \cite{DBLP:journals/csur/Navarro01} on the translation output.
Compared to the standard transformer model, the main difference in terms of the model architecture is that, on top of the transformer decoder blocks, it has two extra prediction heads\footnote{A prediction head is generally implemented as one or more linear layers that take the decoder state as the input.} that predict editing actions for this iteration, namely the \emph{deletion head} $\vec{A}_{del}$ and \emph{mask insertion head} $\vec{A}_{ins}$.
A standard transformer model, on the other hand, only has one prediction head that predicts the upcoming word, which we call \emph{word prediction head} $\vec{A}_{w}$.
At inference time, LevT takes the source sentence and the previous iteration target sequence (or empty sequence for the first iteration) as the input, and applies edits in the order of deletion $\rightarrow$ mask insertion $\rightarrow$ word insertion to generate the sequence iteratively, as shown in Figure~\ref{fig:ter-exp}b.
At training time, the three prediction heads $\vec{A}_w$, $\vec{A}_{del}$ and $\vec{A}_{ins}$ are trained with imitation learning, with the randomly noised target sentence as target-side input and LCS edits as the expert policy.
Like many other non-autoregressive translation models \cite[][\emph{inter alia}]{DBLP:conf/iclr/Gu0XLS18,ghazvininejad-etal-2019-mask,lee-etal-2020-iterative}, LevT also requires training on knowledge distillation data to achieve the optimal performance.
We refer the readers to Appendix \ref{sec:levT-details} and \citet{DBLP:conf/nips/GuWZ19} for details about the model, training scheme, and translation results.

% Levenshtein Transformer \cite[LevT,][]{DBLP:conf/nips/GuWZ19} is a neural network architecture that can iteratively generate sequences in a non-autoregressive manner.
% Unlike normal autoregressive sequence models that have only one prediction head $A_{w}$ to predict the next output words, LevT has two extra prediction heads $A_{del}$ and $A_{ins}$ that predicts deletion and insertion operations based on the output sequence from the previous iteration.
% We now briefly describe the way LevT generates translations, and then the way we use LevT for word-level QE.
% 
% For translation generation, at the $k$-th iteration during decoding, with source-side input $\vec{x}$ and target-side sequence input from the previous iteration $\vec{y}^{(k-1)}$ of length $J$, suppose the decoder block output is $\{\vec{h_0}, \vec{h_1}, \ldots, \vec{h_J}\}$.
% The following predictions and edits will take place in order:
% \begin{itemize}
% 	\item deletion actions $d_j\in\mathcal{D}^{(k)}$: $$p_{del}^{(k)}(d_j\mid\vec{x}, \vec{y}^{(k-1)}) = \text{softmax}(\vec{A}_{del}^T\,\vec{h_j})$$ for $j\in 1\ldots J_0$ and $J_0 = \left|\vec{y}^{(k-1)}\right|$
% 	\item mask insertion actions $\gamma_j\in\mathcal{S}^{(k)}$: $$p_{ins}^{(k)}(\gamma_j\mid\vec{x}, \vec{y}') = \text{softmax}(\vec{A}_{ins}^T\,[\vec{h_j}; \vec{h_{j+1}}])$$ for $j\in 0\ldots J_1$, $\vec{y}'=\mathcal{D}^{(k)}(\vec{y}^{(k-1)})$ and $J_1 = \left|\vec{y}'\right|$
% 	\item word prediction actions $w_j\in\mathcal{W}^{(k)}$: $$p_{w}^{(k)}(w_j\mid\vec{x}, \vec{y}'') = \text{softmax}(\vec{A}_w^T\,\vec{h_j})$$ for $j\in 1\ldots J_2$, $\vec{y}''=\mathcal{S}^{(k)}(\mathcal{D}^{(k)}(\vec{y}^{(k-1)}))$ and $J_2 = \left|\vec{y}''\right|$
% \end{itemize}
% In the end, $\vec{y}^{(k)} = \mathcal{W}^{(k)}(\mathcal{S}^{(k)}(\mathcal{D}^{(k)}(\vec{y}^{(k-1)})))$.
% The iterative process will continue until $\vec{y}^{(k)} = \vec{y}^{(k-1)}$ or a maximum number of iterations is reached.
% 
% For the word-level QE task, we only perform one iteration of the above process -- we use the word deletion head $A_{del}$ to predict quality labels for MT words and the mask insertion head $A_{ins}$ to predict quality labels for gaps.
% We perform neither the word prediction with $A_w$ nor multiple iterations of prediction.
% Still, one should note the similarity between the function of those prediction heads for translation prediction and for word-level QE, which is our motivation for choosing this specific architecture for word-level QE.

\subsection{System Building Process}

\paragraph{Stage 1: Training LevT for Translation}
We largely follow the same procedure as \citet[LevT,][]{DBLP:conf/nips/GuWZ19} to train the LevT translation model, except that we initialize the embedding, the encoder, and decoder of LevT with those from the small M2M-100 model \cite[418M parameters,][]{DBLP:journals/corr/abs-2010-11125} to take advantage of large-scale pretraining.
Because of that, we also use the same sentencepiece model and vocabulary as the M2M-100 model.

For to-English language pairs, we explored training multi-source Levenshtein Transformer model. According to the results on devtest data, this is shown to be beneficial for the QE task for ro-en, ru-en and ne-en, but not for the other language pairs.

\paragraph{Stage 2: Synthetic Finetuning}
During both finetuning stages, we update the model parameters to minimize the NLL loss of word quality labels and gap quality labels, for $\vec{A}_{del}$ and $\vec{A}_{ins}$ respectively.
For language pairs with high translation quality, the translation errors are often quite scarce, thus creating a skewed label distribution over the \texttt{OK} and \texttt{BAD} labels.
To ensure that the model captures both label categories in a balanced manner, we introduce a multiplicative label balance factor $\sigma$ to up-weight the NLL loss of the \texttt{BAD} labels.

To obtain training targets for finetuning, we need \emph{translation triplet data}, i.e. aligned triplet of source, target, and post-edited segments.
Human post-edited data naturally provides all three fields of the triplet, but only comes in a limited quantity.
To further help the model to generalize, we conduct an extra step of finetuning on synthetic translation triplets, similar to some previous work \cite[][\textit{inter alia}]{lee-2020-two}.
We explored six different methods for data synthesis, namely:
\begin{enumerate}
	\item \textbf{src-mt-tgt}: Take the source side of a parallel corpus (\textbf{src}), translate it with a MT model to obtain the MT output (\textbf{mt}), and use the target side of the parallel corpus as the pseudo post-edited output (\textbf{tgt}).
	\item \textbf{src-mt1-mt2}: Take a corpus in the source language (\textbf{src}) and translate it with two different MT systems that have a clear system-level translation quality ordering. Then, take the inferior MT output as the MT output in the triplet (\textbf{mt1}) and the better as the pseudo post-edited output in the triplet (\textbf{mt2}).
	\item \textbf{bt-rt-tgt}: Take a corpus in the target language (\textbf{tgt}) and back-translate it into the source langauge (\textbf{bt}), and then translate again to the target language (\textbf{rt}). We then use \textbf{rt} as the MT output in the triplet and \textbf{tgt} as the pseudo post-edited output in the triplet.
	\item \textbf{bt-noisy-tgt}: Take a corpus in the target language (\textbf{tgt}) and back-translate it into the source language (\textbf{bt}). We then randomly mask some words in the target and let a LevT translation model complete the translation by referring to the \textbf{bt} and masked \textbf{tgt}, which will generate a noisy target sentence (\textbf{noisy}). We then use \textbf{noisy} as the MT output in the triplet and the original target sentence in the corpus (\textbf{tgt}) as the pseudo post-edited output in the triplet.
	\item \textbf{src-rt-ft}: Take a parallel corpus and translate its source side and use it as the pseudo post-edited output (\textbf{ft}), and round-trip translate its target side (\textbf{rt}) as the MT output in the translation triplet.
	\item \textbf{multiview pseudo post-editing (MVPPE)}: This method is inspired by \citet{thompson-post-2020-paraphrase}, which used a multilingual translation system as a zero-shot paraphraser. We take a parallel corpus and translate the source side (\textbf{src}) with a multilingual translation system (\textbf{mt}) as the MT output in the triplet. We then generate the pseudo-post-edited output by ensembling two different \emph{views} of the same model: (1) using the multilingual translation model as a translation model, with \textbf{src} as the input; (2) using the multilingual translation model as a paraphrasing model, with \textbf{tgt} as the input. The ensemble process is the same as standard MT model ensembles and beam search is performed on top of the ensemble.
\end{enumerate}

\RestyleAlgo{ruled}
\begin{algorithm}[t]
 \KwIn{subword-level token sequence $\vec{y}^{sw}$, word-level token sequence $\vec{y}^w$, subword-level tag sequence $\vec{q}^{sw}$}
 \KwOut{word-level tag sequence $\vec{q}^w$}
 $\vec{q}^w \leftarrow$ []\;
 \For{each word $w_k$ in $\vec{y}^w$}{
    find subword index span $(s_k, e_k)$ in $\vec{y}^{sw}$ that corresponds to $w_k$\;
    $\vec{q}^{sw}_{k} \leftarrow$ subword-level translation and gap tags within span $(s_k, e_k)$\;
    $g^{sw}_{s_k} \leftarrow$ subword-level gap tag before span $(s_k, e_k)$\tcp*{$g^{sw}_{s_k-1}\in\vec{q}^{sw}$}
    \eIf{$\forall\,\vec{q}^{sw}_k$ are \texttt{OK}}{
        $\vec{q}^w$ += [$g^{sw}_{s_k}$, \texttt{OK}]\;
    }{
        $\vec{q}^w$ += [$g^{sw}_{s_k}$, \texttt{BAD}]\;
    }
 }
 $\vec{q}^w$ += [$\vec{q}^{sw}$[-1]]\tcp*{add ending gap tag}
 \Return{$\vec{q}^w$}\;
 \caption{Conversion of subword-level tags to word-level tags\label{algo1}}
\end{algorithm}

\paragraph{Stage 3: Human Post-editing Finetuning}
We follow the same procedure as the synthetic finetuning stage except that we finetune on the human post-edited triplet dataset provided by the shared task organizers for this stage.

\subsection{Compatibility With Subwords}

\RestyleAlgo{ruled}
\begin{algorithm}[htbp]
 \KwIn{subword-level token sequence $\vec{y}^{sw}$, word-level token sequence $\vec{y}^w$, naive subword-level tag sequence $\vec{q}^{sw}$, word-level tag sequence $\vec{q}^{w}$}
 \KwOut{heuristic subword-level tag sequence $\widetilde{\vec{q}^{sw}}$}
 $\widetilde{\vec{q}^{sw}} \leftarrow$ []\;
 \For{each word $w_k$ in $\vec{y}^w$}{
   find subword index span $(s_k, e_k)$ in $\vec{y}^{sw}$ that corresponds to $w_k$\;
   $\vec{q}^{sw}_k \leftarrow$ subword-level translation and gap tags within span $(s_k, e_k)$\;
   $t^w_k \leftarrow$ word-level translation tag for $w_k$\tcp*{$t^w_k\in\vec{q}^w$}
   $g^w_k \leftarrow$ word-level gap tag before $w_k$\tcp*{$g^w_k\in\vec{q}^w$}
   $\widetilde{\vec{q}^{sw}}$ += [$g^w_k$]\tcp*{copy left gap tag}
   $n$ = $\left|\vec{q}^{sw}_k\right|$\tcp*{\# subwords for $w_k$}
   \uIf{$t^t_k$ is \texttt{OK}}{
     \tcc{word is \texttt{OK}, so all subwords and gaps between them should be \texttt{OK}}
     $\widetilde{\vec{q}^{sw}}$ += [\texttt{OK}] * $(2n-1)$
   }
   \uElseIf{$\exists\,$\texttt{BAD} in $\vec{q}^{sw}_k$}{
     \tcc{no conflict between subword-level tag and word-level tag -- copy $\vec{q}^{sw}_k$ as-is}
     $\widetilde{\vec{q}^{sw}}$ += $\vec{q}^{sw}_k$\;
   }
   \uElse{
     \tcc{subword-level tag disagrees with word-level tag -- force it as all-\texttt{BAD} to guarantee perfect conversion}
     $\widetilde{\vec{q}^{sw}}$ += [\texttt{BAD}] * $(2n-1)$
   }
 }
 $\widetilde{\vec{q}^{sw}}$ += [$\vec{q}^{w}$[-1]]\tcp*{add ending gap tag}
 \Return{$\widetilde{\vec{q}^{sw}}$}\;
 \caption{Construction of heuristic subword-level tags\label{algo2}}
\end{algorithm}

To the best of our knowledge, previous work on word-level quality estimation either builds models that directly output word-level tags~\cite{lee-2020-two,hu-etal-2020-niutrans-system,moura-etal-2020-ist} or uses simple heuristics to re-assign word-level tags to the first subword token~\cite{wang-etal-2020-hw}.
Since LevT predicts edits on a subword-level starting from translation training, we need to: (1) for inference, convert subword-level tags predicted by the model to word-level tags for evaluation, and (2) for both finetuning stages, build subword-level reference tags.

For inference, the conversion can be easily done by heuristics, as shown in Algorithm \ref{algo1}.
For finetuning, a \emph{naive subword-level tag reference} can be built by running TER alignments on MT and post-edited text after subword tokenization.
However, a preliminary analysis shows that such reference introduces a 10\% error after being converted back to word-level.
Hence, we introduce another heuristic to create \emph{heuristic subword-level tag references}, shown in Algorithm \ref{algo2}.
The high-level idea is to interpolate the word-level and the naive subword-level references to ensure that the interpolated subword-level tag reference can be perfectly converted back to the word-level references.

\subsection{Ensemble}
For each binary label prediction made by the model, the model will give a score $p(\texttt{OK})$, which will be translated into binary labels in post-processing.
To ensemble predictions from $k$ models $p_1(\texttt{OK}), p_2(\texttt{OK}), \dots, p_k(\texttt{OK})$, we perform a linear combination of the scores for each label:
$$p_E(\texttt{OK}) = \lambda_1 p_1(\texttt{OK}) + \lambda_2 p_2(\texttt{OK}) + \dots + \lambda_k p_k(\texttt{OK})$$
To determine the optimal interpolation weights, we optimize towards target-side MCC on the development set.
Because the target-side MCC computation is not implemented in a way such that gradient information can be easily obtained, we experimented with two gradient-free optimization method: Powell method \cite{DBLP:journals/cj/Powell64} and Nelder-Mead method \cite{DBLP:journals/cj/NelderM65}, both as implemented in \texttt{SciPy} \cite{2020SciPy-NMeth}.
We found that Nelder-Mead method tends to find better optimum on the development set while also leading to better performance on the devtest dataset (not involved in optimization).
Hence, we use the Nelder-Mead optimizer for all of our final submissions with ensembles.

